From Daily Song to Daily Self: Supporting Reflective Songwriting of Deaf and Hard-of-Hearing Individuals through Generative Music AI

The rapid advancement of generative AI (GenAI) is expanding access to songwriting, offering a new medium of self-expression for Deaf and Hard-of-Hearing (DHH) individuals. However, emerging technologies that support DHH individuals in expressing themselves through music have largely been evaluated in single-session settings and often fall short in helping users unfamiliar with songwriting convey personal narratives or sustain engagement over time. This paper explores songwriting as an extended, music-based journaling practice that supports sustained emotional reflection over multiple sessions. We introduce SoulNote, a GenAI system enabling DHH to engage in iterative songwriting. Grounded in user-centered design, including a design workshop, a preliminary study, and a multi-session diary study, our findings show that ongoing songwriting with \textit{SoulNote} facilitated emotional growth across three dimensions: self-insight, emotion regulation, and \revised{everyday attitudes toward emotions and self-care}. Overall, this work demonstrates how GenAI can support marginalized communities by transforming creative expression into a daily practice of self-discovery and reflection.

==> Sections/3_Co-design_Workshop.tex <==
As GenAI becomes more prevalent in mental health due to its accessibility and user-centered design, effective clinical use requires customization based on therapeutic domains, user needs, and goals. Co-design with therapists is essential to ensure both usability and clinical relevance \cite{Taewan2024, Inhwa2025}. At the same time, because LLM-based CAs may generate inconsistent or harmful content that compromises therapeutic safety, domain-informed dialogue flow designs are critical for responsible and effective integration into psychotherapy \cite{Dasom2024, Kong2025}.

To address these challenges, we adopted a co-design approach with professional music therapists to explore the use of music from a psychotherapy perspective. DHH users were not included in this initial phase, as the primary aim was to translate established therapeutic techniques into a structured framework for the tool. We first conducted individual interviews with six music therapists to examine the current state of music psychotherapy for DHH clients and to identify needs for supportive tools (section~\ref{individual interview}). Subsequently, we collaborated with four therapists in a creative design workshop to co-develop the therapeutic process and define the core functionalities of a GenAI-assisted music psychotherapy tool (section~\ref{co-design workshop}).

\subsection{Individual Interviews}
\label{individual interview}
\subsubsection{Interview Design}\hfill

\textbf{Participants.} \revised{To address RQ1 on the current state of music psychotherapy practices for DHH individuals, we} first conducted individual interviews with six licensed music therapists who had experience working with DHH clients. Eligible participants were required to have (1) over five years of clinical experience and (2) a relevant professional qualification, such as licensure in counseling or a doctorate in clinical psychology. Therapists without prior experience working with DHH clients were excluded because music therapy for DHH individuals demands specialized knowledge and protocols tailored to their unique sensory and emotional characteristics. Therefore, recruiting qualified participants was challenging \cite{ward2016, Palmer2022}; therefore, six participants were recruited for this study. All therapists were recruited via professional networks and referrals from therapeutic centers. All participants identified as female. Their age (M=36.5, SD=3.78) and years of experience (M=7.83, SD=2.78) are presented in (Table~\ref{tab: population}). Each therapist had worked with a broad range of DHH clients, from children to older adults. While their primary field was music perception, some also incorporated music psychotherapy in clinical contexts. All participants were familiar with GenAI tools such as ChatGPT \footnote{https://chatgpt.com/} and had hands-on experience using LLM-based CAs or music GenAI systems like SUNO\footnote{https://suno.com/}. Before the interviews, participants completed a demographic survey and provided written consent. The study was approved by the Institutional Review Board (IRB) at [anonymized university], Korea.

\begin{table*}[t]
\begin{center}
\caption{Demographic information of the individual interview and design workshop}
  \label{tab: population}
  \begin{tabular}{c|c|c|c|c|c|c|c|c}
    \toprule
    \multirow{2}{*}{ID} & \multirow{2}{*}{Gender} & \multirow{2}{*}{Age} & \multirow{2}{*}{Job title} & \multirow{2}{*}{Specific field} & Years of & \multicolumn{2}{c|}{Participation} & \multirow{2}{*}{\revised{Knowledge of GenAI}}\\
    \hhline{~~~~~~--|~}
    &&&&& experience & Interview & DW & \\
    \midrule
    T1 & Female & 40 & Clinical music therapist & Percept (Psycho) & 11 & O & O & Experienced\\
    T2 & Female & 32 & Licensed music therapist & Percept (Psycho) & 5 & O & O & Experienced\\
    T3 & Female & 35 & Licensed music therapist & Percept (Psycho) & 6  & O & O & Experienced\\
    T4 & Female & 36 & Licensed music therapist & Percept (Psycho) & 10 & O & O & Knowledge\\
    T5 & Female & 42 & Clinical music therapist & Percept & 10 & O &  - & Experienced\\
    T6 & Female & 34 & Licensed music therapist & Percept & 5 & O & - & Knowledge\\
    \bottomrule
    \multicolumn{9}{>{\raggedright\arraybackslash}p{\dimexpr\linewidth-2\tabcolsep\relax}}{\small Job title: someone who holds a music therapy-related license (Licensed music therapist) and either has a doctoral degree as a clinical music therapist (Clinical music therapy); Specific field: primarily music perception (Percept), with additional experiences in music psychotherapy (Psycho); Participation: interview and design workshop (DW); \revised{GenAI: prior usage (Experienced) and awareness only (Knowledge)}.}
\end{tabular}
 \vspace{-10pt}
\end{center}
\end{table*}

\textbf{Process.} We conducted 60-minute semi-structured interviews focused on two main topics: (1) the current state of music psychotherapy for DHH clients, and (2) the practical needs and challenges in this domain (see Appendix~\ref{adx: interview details} for more details). With consent, all sessions were recorded and transcribed. Two researchers independently coded the transcripts by categorizing data into three themes: therapeutic context, challenges, and support needs using thematic coding \cite{Virginia2006}. After two rounds of discussion, the coding was refined, and the following two key findings were identified.

\subsubsection{Findings. Current Practices and Needs in Music Psychotherapy for DHH individuals \revised{(RQ1)}} \hfill

\textbf{Therapeutic priorities shaped by constraints of time and cost.} 
Therapists reported that most DHH clients prioritize music perception training aimed at improving auditory function over long-term emotional healing, largely due to constraints in time, cost, and accessibility. These limitations were especially pronounced among adult clients, who often favored short-term, results-oriented auditory training. Many believed that improving their auditory perception through music-based training would naturally resolve their social and emotional difficulties. 

\begin{quote}
\textit{``From the client’s perspective, recovering auditory function is observed as the top priority. Emotional therapy often gets pushed aside, especially for adults who are constrained by time and cost due to work or life responsibilities.''} (T1)
\end{quote}
\begin{quote}
\textit{``Adults tend to be reluctant to invest in emotional therapy. They want to feel their time and money were well spent—usually through functional outcomes.''} (T4)
\end{quote}

However, therapists noted that while perception-based approaches had functional benefits, they often failed to address underlying emotional needs. Hearing loss is often described as a \textit{“hidden disability,”} contributing to frequent misunderstandings and feelings of exclusion among DHH individuals. Therapists unanimously noted that their DHH clients frequently struggled with chronic emotional issues, including low self-esteem and depression. Even when their auditory perception improved through training, therapists consistently observed symptoms of depression, anxiety, and stress rooted in social isolation or unresolved trauma. Even with improved auditory skills, many clients continued to experience emotional distress and lacked confidence in social settings.
\begin{quote}
\textit{``Even after regaining some hearing ability, many clients carry self-defeating beliefs like `I’m still not good enough.' It’s like treating a car accident injury without addressing the trauma.''} (T6)
\end{quote}

\textbf{Symbolic significance of music to DHH individuals and the lack of tailored psychotherapy tools.} To address this, four therapists integrated songwriting into treatment alongside perception training, using music and lyrics as tools for emotional expression and self-reflection. They shared examples where songwriting enables clients to express internal struggles and rebuild confidence. However, therapists noted challenges in consistently applying songwriting, especially with adult clients facing a shorter treatment window. While therapists sought remote or digital solutions to extend emotional support outside of sessions, they emphasized the lack of therapy systems that account for the unique sensory and communicative characteristics of DHH individuals. In particular, emotional engagement through music listening remains constrained for many DHH clients, underscoring the need for more accessible and multimodal systems. All therapists emphasized the need for accessible and flexible systems to support emotional healing through music, especially for DHH individuals facing practical and emotional barriers to in-person care. 
\begin{quote}
\textit{``With a postlingual hearing loss client, we used song discussion for about three months. Eventually, they shared that colleagues noticed he looked more cheerful and spoke more confidently at work.''} (T2)
\end{quote}
\begin{quote}
\textit{``There are many clients who can’t afford therapy or avoid social interactions, so we need remote-access tools. But emotional therapy systems are nearly non-existent compared to music perception tools.''} (T3)
\end{quote}


\subsection{Co-design Workshop}
\label{co-design workshop}
Insights from interviews revealed key challenges in DHH music psychotherapy: cost constraints and insufficient systemic support. These barriers often prevent consistent access to psychotherapeutic services, especially without the presence of a therapist. To address this gap, we explored the potential of a GenAI-assisted music psychotherapy support tool that could offer greater flexibility and accessibility. We conducted a co-design workshop with four of them to explore a GenAI-based intervention. \cite{Norman1986}.

\subsubsection{Participants and Process}
\hfill

\textbf{Participants.} The co-design workshop \revised{included} practicing therapists at an early stage of the design process, ensuring that the GenAI tool reflects therapeutic perspectives while addressing the needs and values of DHH users.  Four music therapists (T1-T4) who had participated in the prior interviews were recruited; they had experience treating DHH clients with anxiety, stress, or depression (Table~\ref{tab: population}). \revised{The lead therapist (T1) was selected from this cohort based on more than ten years of clinical work with DHH clients and prior hands-on experience with LLM-based CAs and music-generation tools, for example, ChatGPT and SUNO. Before data collection, we held a 30-minute preparation session with the lead therapist to review the workshop goals, ethical considerations, and risk-management procedures. Because therapists differed in familiarity with GenAI, we ran a brief hands-on exercise using ChatGPT and SUNO for all participants and collected short written reflections on perceived affordances prior to the main ideation activities.} 

\textbf{Process.} Following user-centered design principles \cite{Norman1986}, we conducted a 4-hour remote workshop comprising five sessions (Figure~\ref{fig: design workshop process}): (1) introduction, (2) persona design, (3) GenAI solution exploration, (4) therapy process design, and (5) debriefing. To tailor the tool to the needs of DHH clients, we employed a persona design approach that allowed therapists to externalize their tacit knowledge and articulate user needs more concretely \cite{Norman1986, Weitz2024}. Participants first created representative personas based on their clinical experiences, grounding the design in real-world therapeutic practice (persona design). They then identified expected challenges in applying GenAI-based interventions to these personas and explored potential solutions (GenAI solution exploration). Finally, they designed concrete therapeutic processes and example prompts incorporating established music therapy techniques (therapy process design). To minimize researcher bias during the workshop, sessions were facilitated by a lead therapist who guided the discussions. The workshop took place over an online video call meeting, and participants collaborated in real time using a shared web-based tool.

Specifically, the design sessions combined individual and group-based activities to balance therapists’ clinical insights with collaborative synthesis \cite{Bodker2009}. The individual design allowed each therapist to work independently, minimizing potential bias from others and encouraging the expression of unique perspectives. In contrast, the group sessions aimed to build a shared understanding and organize key themes while preserving the richness of each therapist’s viewpoint, as illustrated in Figure~\ref{fig: design workshop process}. In the persona design session, each therapist independently created a DHH client persona. The group then collaboratively synthesized these into two representative personas and discussed the anticipated challenges and opportunities for applying GenAI technologies for each persona. Following this, participants individually designed the process and example prompts for a GenAI-assisted music psychotherapy tool. These designs were then refined through group discussion to finalize the therapeutic framework. Details of the procedure are provided in the Appendix~\ref{adx: design workshop}.


\subsubsection{Material and Analysis}
\hfill

\textbf{Material.} We used shared Google documents\footnote{https://docs.google.com/} for collaboration, including a persona worksheet and a therapy flowchart template. The persona worksheet included demographics, hearing status, musical background, and therapeutic goals. The flowchart sheet structured the therapy process step by step, based on each persona’s characteristics (Figure \ref{fig: AppendixA}-A in Appendix). Before the workshop, participants received an overview and practice guide to familiarize themselves with the GenAI tools, including ChatGPT to illustrate the concept of a CA and SUNO to demonstrate the capabilities of language-based music GenAI.

\textbf{Data Collection and Analysis.} Data were collected through video recordings, digital worksheets, and researcher field notes. Two researchers observed the sessions and used open-ended format sheets to document their observations. All verbal data were transcribed and analyzed thematically to identify core themes and recurring patterns \cite{Virginia2006}. Predefined codes, based on field note parameters, guided the analysis, which focused on informing prototype design through a nuanced understanding of DHH client characteristics. The lead therapist and two researchers collaboratively analyzed two discussion sessions, identifying the key characteristics of the DHH clients, appropriate GenAI strategies, and a detailed system process.

\begin{figure*}[ht]
  \centering
  \includegraphics[width=1\textwidth]{Figures/workshop.png}
  \caption{Design workshop process. Sessions comprise persona design, a discussion about GenAI-based technology, and process design. In the design session, the final design emerged from group discussion, led by the main facilitator (T1, red), after individual design work.}
  \label{fig: design workshop process}
\end{figure*}


\subsection{\revised{Findings, Design Rationale, and Therapy Process Design}}

\revised{To address RQ2 on the design rationale of a GenAI-assisted songwriting tool for DHH music psychotherapy, we conducted a co-design workshop with practicing music therapists.} Through the workshop, we identified the representative characteristics and expected challenges of DHH clients commonly encountered by therapists (persona design session), explored potential strategies involving CA and music GenAI to address these challenges (GenAI solution exploration session), and developed concrete therapeutic processes and example questions incorporating music therapy techniques (therapy process design session). From these processes, the identified characteristics of DHH and the corresponding GenAI strategies are as follows. \revised{Based on these processes, we derive the following design rationales, expressed as pairs of DHH client characteristics and corresponding GenAI strategies.}

\subsubsection{\revised{Findings: Characteristics and Challenges of DHH individuals}}\hfill


\textbf{\revised{Finding 1. Communication barriers and social isolation.}} 
\phantomsection  %
\label{finding:1}
During the persona design sessions, the four therapists synthesized two representative personas, A and B, from the common characteristics of DHH individuals observed in the individual personas (Table~\ref{tab: persona}). Both A and B were described as DHH individuals who were either preparing for employment or currently unemployed, experiencing social anxiety and challenges in self-expression. The therapists clarified that these personas were not intended to generalize all DHH individuals but rather to capture common patterns observed among clients seeking emotional support or psychotherapy. They explained their depiction of personas A and B as socially isolated DHH people by noting that communication difficulties associated with hearing loss often manifest as emotional consequences in daily life and interpersonal relationships. In practice, they concurred that many clients displayed such tendencies, including introversion, reservation, difficulties in social participation, and occasional avoidance of social interactions. From their empirical observations, therapists noted that these characteristics of DHH clients could hinder personal expression in songwriting-based music therapy, sometimes leading individuals to adopt defensive or withdrawn attitudes that delayed the process.

\textbf{\revised{Finding 2. Negative sound-related experiences and low confidence in songwriting.}} 
\phantomsection  %
\label{finding:2}
Another shared characteristic of personas A and B was a lack of confidence in sound-related activities. Although they had some experience with music listening, they had little to no experience in songwriting and were described as exhibiting a passive attitude due to low confidence in engaging with sound (Table~\ref{tab: persona}). Therapists reported that DHH clients often experienced a lack of confidence in songwriting stemming from negative past experiences with sound-related activities (e.g., \textit{singing classes or presentations}). They agreed that this lack of creative confidence served as a barrier to therapeutic engagement. Moreover, insufficient confidence in music was considered likely to hinder not only the initiation of songwriting but also its capacity to serve as a means of sustaining ongoing self-expression.


\begin{table*}[t]
\begin{center}
  \caption{Two DHH clients' personas designed from the design workshop}
  \label{tab: persona}
  \begin{tabular}{C{3cm}|C{7cm}|C{7cm}}
    \toprule
    & Persona A. Kim (Male, 26) & Persona B. Choi (Female, 40) \\
    \midrule
    Occupation & Job seeker & Homemaker on career break for childcare \\
    \hline
    Hearing Status & Hearing loss (Innate) & Hearing loss (Infant) \\
    \hline
    Personality & Closed, introverted & Closed, introverted \\
    \hline
    Interaction	& Limited in peer relationships and interactions due to hearing impairment & Difficulty communicating with children and husband due to hearing loss \\
    \hline
    Motivation & Treating fear of social interaction for social activities & Feeling socially isolated due to career interruption and hearing loss, expressing depression and helplessness \\
    \hline
    Purpose & Improving confidence through positive sound experiences for smooth interpersonal relationships and interactions & Confronting personal situation and discovering inner resources (strengths) \\
    \hline
    Music Experience & Various educational experiences including instrument playing beyond regular music education & None music experience beyond regular education \\
    \hline
    Music Preference & Various music genres & Limited music preferences \\
    \hline
    Anticipated Challenges & Expected difficulty expressing personal situation and challenges & Low motivation for the treatment process and difficulty completing music due to helpless state \\
    \bottomrule
\end{tabular}

 \vspace{-10pt}
\end{center}
\end{table*}


\subsubsection{\revised{Design Rationale for a GenAI-assisted Songwriting Tool} \revised{(RQ2)}}\hfill

\revised{Building on these findings, we derived the following design rationales for a GenAI-assisted songwriting tool that supports DHH individuals in music psychotherapy.}

\textbf{DR1. Supportive conversational strategies are needed to facilitate emotional expression.} \revised{Based on \hyperref[finding:1]{Finding 1},} therapists anticipated that DHH users would experience difficulties in directly expressing their emotions and challenges to a CA. Accordingly, during the GenAI solution exploration session, they discussed strategies to address this issue and proposed two key approaches: \textit{supportive empathy} and \textit{multiple example response options}. First, similar to how therapists empathize with clients’ psychological distress and help them regain emotional balance, the CA was considered to require supportive and empathetic responses that encourage DHH individuals to express themselves. They also emphasized that, given the need for safety when discussing negative situations, the CA’s interventions should remain at a foundational supportive-level approach typical of music therapy \cite{cadesky2006music}. This would ensure that music functions as a safe and constructive medium, helping clients to identify the structures and resources necessary to address personal difficulties. Providing supportive empathy for the user’s current state was regarded as essential to fostering emotional openness, especially for DHH users who may initially display emotional reticence. Second, to accommodate DHH users who may face challenges in verbal expression, the therapists suggested incorporating selectable response options alongside questions to facilitate more flexible and accessible interactions. For example, since DHH users may struggle with naming their emotions in specific contexts, presenting a set of emotion-related keywords for users to choose from was considered an important strategy. 


\textbf{DR2. Independent songwriting experiences are needed.} 
\revised{Drawing on  \hyperref[finding:2]{Finding 2},} therapists suggested that music GenAI could reduce the burden of songwriting and enhance clients’ confidence and creative motivation by enabling them to rapidly experiment with lyrics and musical structures. However, they emphasized the importance of ensuring that DHH users perceive the resulting songwriting as their own. In this regard, maintaining clients’ agency and choice throughout the songwriting process was considered essential. To achieve this agency, it is necessary to elicit musical expressions that reflect the characteristics of DHH users. Therapists mentioned that, being accustomed to visually oriented language, DHH individuals are often adept at describing visual scenes. They therefore proposed that structuring narratives around clients’ situations in an image-based approach could facilitate the expression of lyrics and musical elements. To this end, they recommended that the CA employ \textit{visual-based metaphors and analogies} to support users in articulating their musical expression, thereby enabling a more accessible and intuitive conversational strategy for songwriting.

\subsubsection{Generative AI-assistive Therapy Process Design}
\label{sec: 3.3.3}
To design songwriting support tools that account for the accessibility and emotional safety of DHH individuals, therapists drew on their existing music therapy practices and outlined four key processes during the therapy process design session: (1) therapeutic connection, (2)  making lyrics, (3) making music, and (4) song discussion (Figure~\ref{fig: process and examples}). The workflow and corresponding question list can be found in Figures~\ref {fig: AppendixA}-B in the Appendix.

\begin{itemize}
    \item \textbf{Therapeutic connection (Figure~\ref{fig: process and examples}A)} Based on the introverted tendencies of DHH clients inferred from the personas, therapists initiate the design process with a rapport-building stage that includes questions about the user’s name, recent emotional experiences, difficult situations they are facing, motivation for songwriting, and musical preferences. At this state, the CA responds with empathy to the user’s emotional expression (\textit{supportive empathy}) and provides (\textit{example response options}) to assist DHH users who may find it difficult to answer questions related to personal challenges. To encourage emotional expression through music, the CA also offers motivational support by highlighting the positive effects of engaging in musical experiences. 
    \item \textbf{Making lyrics (Figure~\ref{fig: process and examples}B)}. As the second state, therapists designed a process in which users collaborate with the CA to write lyrics. Based on emotional themes identified earlier, the CA prompts discussion on the purpose and concept of the musical piece. In particular, for users who struggle with lyrics writing, the CA encourages DHH users to visualize and describe situations, emotional expressions, and contextual scenes related to their personal challenges through \textit{visual-based metaphor and analogy}. For highly engaged users, the CA was designed to encourage them to initiate the lyrics by writing the first line themselves, thereby reinforcing their sense of authorship and immersion. 
    \item \textbf{Making music (Figure~\ref{fig: process and examples}C)}. Based on the music GenAI system (SUNO), therapists designed the process so that users could select musical attributes—genre, mood, instrumentation, vocal style, melody, and rhythm—based on personal preference and emotional context. Therapists highlighted the importance of having the CA suggest musical elements that reflect the user's intended concept and offer customized options to assist users with limited songwriting experience in navigating the selection process with \textit{example response options}. Therapists also emphasized that translating musical elements into visual representations through music analysis (e.g., \textit{lyrics animation}) is essential for supporting emotional engagement, as it enables DHH users to better perceive and appreciate the musical experience. This approach provides visually accessible and emotionally meaningful feedback, thereby enhancing user engagement.
    \item \textbf{Song discussion (Figure~\ref{fig: process and examples}D)}. Therapists highlighted that initiating a reflective dialogue following songwriting is a crucial role of the CA, as it facilitates emotional insight, self-reflection, and deeper engagement with the therapeutic value of music. The CA proceeds to reflective prompts such as \textit{“Was there a particular part of the song that resonated with you?”} to guide the user in interpreting the emotional significance of the work. This final state supports deeper self-awareness and therapeutic insight, transforming the tool from a creative platform into one for emotional exploration and psychological healing.
\end{itemize}



\begin{figure*}[ht]
  \centering
  \includegraphics[width=1\textwidth]{Figures/process.png}
  \caption{States and representative Q\&A examples of the music psychotherapy assistive tool. The process consists of four states: Therapeutic connection (A), Making lyrics (B), Making music (C), and Song discussion (D). Each state contains the steps and required variables that serve as the criteria for proceeding to the next state. Examples of the CA's three conversational strategies are indicated using color coding - supportive empathy (pink), example response option (green), and visual-based metaphor and analogy (yellow).}
  \label{fig: process and examples}
\end{figure*}


==> Sections/6_Collaborative_Songwriting.tex <==
\subsection{Reflective Songwriting Interaction based on Personal Challenges}
\label{sec: 6.1}

Our results section is organized around three key findings.
First, all participants expressed their struggles and current emotional states through conversations with the CA, during which they collaboratively completed the songwriting process (Section \ref{sec: 6.1}).
Second, we identified specific strengths of the CA and conversational strategies that enhanced the participants' songwriting experiences (Section \ref{sec: 6.2}).
Third, we observed the potential therapeutic effects of songwriting, highlighting its value as a process for emotional healing (Section \ref{sec: 6.3}).

\subsubsection{Overall Usage.} Figure~\ref{fig: use pattern} shows the time participants spent in each songwriting state. All participants completed their songwriting sessions without discontinuity. The average total usage time was 40.15 minutes (SD=10.08). Questionnaire responses on system usability (Figure~\ref{fig: result}A) also showed high ease of use. Most participants reported that using the proposed tool did not require significant effort or impose any noticeable burden. Therapist monitoring confirmed that no participant exhibited signs of emotional distress or negative reinforcement during CA interaction. Most users remained calm, emotionally neutral, and engaged.

\begin{figure*}[ht]
  \centering
  \includegraphics[width=0.8\textwidth]{Figures/usePattern.png}
  \caption{Individual time spent by participants in each songwriting state. Participants spent an average of 5.07 minutes (SD=3.00) building rapport with the CA, followed by 13.13 minutes (SD=8.59) discussing lyrics and 14.40 minutes (SD=7.17) discussing musical elements such as genre. They then spend 7.55 minutes (SD=5.56) sharing thoughts and emotions about the generated music.}
  \label{fig: use pattern}
\end{figure*}

\subsubsection{Initial Personal Challenges and Music Concepts.} During the co-design workshop, therapists anticipated that DHH clients might struggle to verbalize emotions or life circumstances due to their typically reserved communication styles. However, as shown in Figure~\ref{fig: result}B, most participants reported little difficulty expressing themselves to the CA. Average scores for self-disclosure were high (M=6.02, SD=1.05), with moderate levels of social presence (M=5.02, SD=1.38). Fear of the CA was relatively low (M=2.94, SD=1.60), and trust in the CA was moderately high (M=4.38, SD=1.37). Participants appeared open to sharing personal experiences and emotions, interacting with the tool in a generally receptive and trusting manner.

Most participants (n=16) shared personal struggles, including social isolation from hearing loss, future-related anxiety, and relationship tensions, in response to the CA’s opening prompt \textit{(``What kinds of thoughts or feelings have you been experiencing lately?'')}. These challenges were grouped into four themes: difficulties communicating with family or colleagues due to hearing loss (\textit{Relationships}, n=7); anxiety about job hunting, financial insecurity, or career transitions (\textit{Life stability}, n=7); loss of meaning or identity after quitting work, or feeling purposeless (\textit{Personal fulfillment}, n=2); emotional states shared without clear situational background (\textit{Non-contextual feelings}, n=5). These reflections served as key motivators for songwriting and helped shape the lyrical themes. Although music concepts were not always directly tied to the specific challenge, most participants pursued songwriting with one of three therapeutic aims: creating music to release emotions or offer comfort in the present (\textit{Emotional relief}, n=9); using lyrics to express and reframe personal experiences (\textit{Emotional acceptance}, n=3); reconnecting with positive memories or relationships to overcome stagnation (\textit{Motivation}, n=11). 

\begin{figure*}[ht]
  \centering
  \includegraphics[width=0.8\textwidth]{Figures/result.png}
  \caption{Questionnaire result: system usability (A), perception of CA (B), and music satisfaction (C) rating 7-point Likert scale by participants, and scores were grouped into six categories: 1–2=strongly disagree, 2–3=disagree, 3–4=slightly disagree, 4–5=slightly agree, 5–6=agree, and 6–7=strongly agree. (*) indicates reversed interpretation direction, where higher and lower agreement reflect a more favorable outcome, in contrast to the other items.}
  \label{fig: result}
\end{figure*}


\subsection{Facilitative Interaction Strategies of CA in Songwriting}
\label{sec: 6.2}
\subsubsection{Facilitating Self-Disclosure}\hfill

\textbf{Psychological safety from being judgment-free.} Most participants (n=22) said they felt more comfortable speaking with the CA than with family, friends, or therapists because a text-based chatbot provided a judgment-free space that was easier to navigate than spoken interaction. Many (n=20) noted that the CA’s inability to perceive external cues, such as appearance or tone of voice, made them feel safer and more willing to share, as some DHH users may feel less confident about how their voice or speaking style is perceived during conversations. Some (n=11) specifically highlighted their trust that the CA would respond empathetically and preserve their confidentiality.

\begin{quote}
\textit{``It was much easier talking to the chatbot than to my family or friends. I felt more relaxed knowing it wouldn’t judge me based on how I look or speak.''} (P1)
\end{quote}
\begin{quote}
\textit{``I felt like I could say anything to the chatbot. I trusted that it wouldn’t judge me or share my words with anyone else.''} (P6)
\end{quote}

\textbf{Emotional acceptance promoting openness.} In line with the \textit{supportive empathy} strategy, we guided the CA’s responses to be supportive and emotionally responsive to users’ input. Fifteen participants said that the CA’s empathetic responses encouraged them to open up. Participants reported experiencing three distinct types of empathetic responses from the CA: (1) mirroring empathy— simply repeating the user’s statements; (2) interpretive empathy— rephrasing the emotional meaning behind what was said; and (3) proactive empathy—acknowledging emotions before they are explicitly expressed (Table~\ref{tab: chat transcript-empathy}). Participants especially appreciated proactive empathy, finding it emotionally resonant and affirming. They noted that, unlike responses that merely mirrored their statements, proactive empathy expressed in the chatbot’s language felt more like genuine comfort, which made the interaction feel more human and emotionally sincere. This mirrors the therapist's \textit{``holding''} technique \cite{cooper2012musical}, where a safe space is maintained through reflective presence. 

\begin{quote}
\textit{``When I said I quit dancing due to hearing loss, it acknowledged that and made me feel understood. I felt the chatbot was really paying attention to me.''} (P7)
\end{quote}
\begin{quote}
\textit{``When I said I got divorced, the chatbot said, ‘You have gone through a tough time,’ and that really got to me.''} (P8)
\end{quote}


\begin{table*}[t]
\begin{center}
  \caption{Chat transcript in our tool: Empathy strategies (Mirroring empathy, Interpretive empathy, Proactive empathy)}
  \label{tab: chat transcript-empathy}
  \begin{tabular}{C{3cm}|C{2cm}|p{11cm}}
    \toprule
    Type of Empathy & Utterer & \multicolumn{1}{c}{Contents}\\
    \midrule
    \multirow{2}{=}{\centering Mirroring \\Empathy (P1)} & User & ``I worry about what if someone thinks badly of me''\\
    \hhline{~--}
    & Bot & ``That must be very concerning for you''\\
    \midrule
    \multirow{2}{2cm}[-0.8ex]{\centering Interpretive Empathy (P6)} & User & ``I want to make people happy, but I'm unable to do it well''\\
    \hhline{~--}
    & \multirow{1}{1cm}[-1.5ex]{\centering Bot}  & ``I understand how challenging it must be to want to make others happy but not feel able to. You really do seem to have such a warm heart''\\
    \midrule
    \multirow{2}{2cm}[-0.8ex]{\centering Proactive Empathy (P7)} & User & ``I quit dancing and deliberately tried to dislike dance''\\
    \hhline{~--}
    & \multirow{1}{1cm}[-1.5ex]{\centering Bot} & ``When you decided to pause dancing, you might have felt a mix of things, perhaps heaviness or a wish to step back''\\
    \bottomrule
\end{tabular}

 \vspace{-10pt}
\end{center}
\end{table*}
 
\textbf{Safe emotional expression through songwriting.} As their personal expressions were transformed into lyrics and music, which reduced the psychological burden of sharing, many participants shared that creating music together with the CA made emotional disclosure feel safer and more natural. Especially, eight participants who initially hesitated to open up noted that the structured nature of songwriting helped them reflect and share more of their experiences. Specifically, the CA’s step-by-step prompts, ranging from option selection and scene description to sentence building and lyrics writing, guided users in understanding their own emotional states and experiences, making the disclosure process feel more approachable and meaningful. They also emphasized that introducing songwriting gradually, rather than at the beginning of the session, helped them feel more emotionally ready and engaged. If they had been asked to create music right away, it might have felt overwhelming; instead, starting from a space of personal sharing allowed them to transition into songwriting in a more motivated and emotionally grounded way.

\begin{quote}
\textit{``Rather than just talking about my feelings with the chatbot, writing lyrics made it easier and even fun to express things I couldn’t say directly.''} (P2)
\end{quote}
\begin{quote}
\textit{``If it had just been a normal chatbot conversation, I might’ve said something like ‘I’m just annoyed’ and left it at that. But through music, I could reflect and express myself more honestly.''} (P4)
\end{quote}

\textbf{Balance between direct questions and natural dialogue.} Most participants (n=17) reported that the CA’s direct questions during the songwriting process facilitated valuable self-reflection and disclosure. They appreciated that when they naturally shared difficult experiences, such as disability or divorce, topics rarely addressed in daily conversations, the CA provided space to talk about them. This process enabled them to articulate personal experiences that had long remained unexpressed.
\begin{quote}
\textit{``The chatbot asked about topics people usually avoid, like disability, and I actually felt more comfortable answering them.''} (P7)
\end{quote}

However, this approach was not universally effective. A smaller group (n=5) found that explicit emotional questions felt psychologically pressuring, \revised{as if the CA were pushing them to confront sensitive issues before they were ready. Because the questions remained quite direct, they noted that they felt obliged to keep responding rather than choosing when and how to share.} These participants preferred a more conversational approach, where emotional sharing would emerge organically through a broader range of topics. Additionally, three participants felt that the CA was overly focused on progressing through the songwriting steps, which made the conversation feel rushed and limited deeper emotional exploration.
\begin{quote}
\textit{``As the questions kept coming, I started feeling pressured to answer. It might feel easier if the chatbot collected this information more casually through conversation.''} (P3)
\end{quote}
\revised{These mixed experiences indicate that future GenAI CAs for psychotherapy should allow users to adjust the directness and pacing of questions, for example, by switching between more structured and more casual conversational modes. They should also include mechanisms that help slow the pace or temporarily shift away from emotionally intense topics when users feel overwhelmed.}

\subsubsection{Facilitating Songwriting Experience}\hfill

All participants completed the songwriting process with the CA, sharing their current circumstances and emotions and using these as guidelines. As shown in Figure~\ref{fig: result}C, satisfaction with the songwriting experience of participants was high (M=5.86, SD=0.94).

\textbf{Music concretization music through visual thinking.} Twenty participants reported that the CA’s visually imaginative prompts helped transform abstract feelings into concrete scenes, easing the lyrics writing process and enhancing emotional articulation (Table~\ref{tab: chat transcript-visual}A, \textit{visual-based questions}). For example, questions such as \textit{``What color best represents your current mood?''} or \textit{``Can you describe a scene or place that reflects how you feel right now?''} encouraged users to translate emotions into vivid sensory imagery. These visual metaphors helped users externalize complex feelings and anchor them in narrative or symbolic forms that could be woven into lyrics.

\begin{quote}
\textit{``Questions like ‘What kind of scene comes to mind?’ really helped. I turned my abstract sadness from divorce into the image of sitting by a rainy window.''} (P8)
\end{quote}
\begin{quote}
\textit{``Describing my job hunt frustration as sitting alone in my room helped me feel like I was escaping that emotional confinement.''} (P12)
\end{quote}

Fourteen participants noted that the CA’s non-technical and intuitive suggestions made musical decision-making more accessible. Instead of relying on technical musical terminology, the CA encouraged users to imagine visual scenes or emotional atmospheres (e.g., \textit{selecting a tempo based on the urgency conveyed in a visual image in their mind}). When explanations linked emotions or narratives to specific choices, participants reported feeling more emotionally engaged in the music-making process (Table~\ref{tab: chat transcript-visual}B, \textit{example response option}). This collaborative framing helped bridge the psychological gap between the user and the GenAI.

\begin{quote}
\textit{``I wasn’t sure whether to choose piano or strings. The chatbot explained, `Piano expresses personal emotions, while strings can add emotional depth.' That explanation helped me pick the instrument that best matched my story. If it had just listed instrument names, I might have chosen randomly, but knowing the meaning made me more emotionally connected to the music.''} (P16)
\end{quote}


\begin{table*}[t]
\begin{center}
  \caption{Chat transcript in our tool: Visual and example-providing conversation strategy (P8)}
  \label{tab: chat transcript-visual}
  \begin{tabular}{C{2cm}|p{14cm}}
    \toprule
    Utterer & \multicolumn{1}{c}{Contents} \\
    \midrule
    Bot & ``You said you wanted to create music about a situation where you felt frustrated but became calm as time passed. \textbf{(A) Do you have any images that come to mind about this topic? (B) For example, the quietness after a storm, or it could be some aspect of nature.}'' \\
    \hline
    User &  ``I'm thinking of the image of rough waves at the seaside. Initially rough, but gradually becoming calm as they approach the sand and break.'' \\
    \hline
    Bot & ``You mentioned wanting to express the transition from rough sea waves to calmness in lyrics. What specific words come to mind when expressing this emotion more concretely? \textbf{(B) For example, words like `rough', `calm', `peaceful' could be used.}''\\
    \hline
    User &  ``Rough, calm, angry, composed.''\\
    \hline
    Bot & ``You said you wanted to express in lyrics that moment when rough waves at the seaside gradually become calm. Using the words `rough', `calm', `angry', and `composed', shall we develop lyrics that initially depict rough waves crashing, then gradually transition to a calmer state? How could we combine these words to create sentences? Or would you like me to provide an example first?''\\
    \hline
    User & ``Returning from the distant sea, the rough waves became calm as they approached the sand. My greatly shaken heart also became composed.''\\
    \hline
    Bot & ``We are starting with the words `rough', `calm', `angry', `composed' and proceeding with lyrics depicting the calming of sea waves. For the beginning part of the lyrics, what scene would be good to start with?''\\
    \hline
    User &  ``I think it would be good to describe waves crashing violently.''\\
    \bottomrule
     \multicolumn{2}{>{\raggedright\arraybackslash}p{\dimexpr\linewidth-2\tabcolsep\relax}}{\small 
     The bold text (A) shows questions based on visual-based metaphor and analogy, and (B) shows a conversation providing examples that participants could refer to when answering.}
\end{tabular}

 \vspace{-10pt}
\end{center}
\end{table*}


\subsection{Emotional Transformation through the Musical Output}
\label{sec: 6.3}
\subsubsection{Emotional Objectification and Personalized Comfort through Lyrics Writing}\hfill

\revised{\textbf{Personal healing compared to commercial lyrics.}} While many participants (n=12) had previously found general solace in commercial lyrics, creating lyrics that directly reflected their own stories provided a stronger sense of healing. Some (n=3) shared that turning difficult experiences into lyrics helped them perceive their situations more objectively. In several cases, emotions that previously felt overwhelming became more manageable, or even humorous, once expressed creatively through song. 

\begin{quote}
\textit{``Listening to music gives general comfort, but writing a song brings personal healing.''} (P2)
\end{quote}

\revised{\textbf{Emotional distancing through self-authored lyrics.}} Notably, most participants (n=15) mentioned that the CA played an important role in this process by prompting users with direct and personalized questions, which encouraged them to reflect on and share stories they might have otherwise avoided. By helping users transform these reflections into lyrics and music, the CA supported emotional distancing and reframing through the externalization of internal states.

\begin{quote}
\textit{``If I had just written it out, I’d have said something like ‘I was annoyed, I was angry.’ But turning it into a humorous song helped me see the situation more clearly.''} (P4)
\end{quote}


\subsubsection{Emotional Transformation and Affective Expansion through Musical Expression}\hfill

\revised{\textbf{Emotional release and expansion through multimodal musical expression.}} Most participants (n=20) reported emotional transformation while listening to the completed music. All participants expressed satisfaction that their interaction with the CA culminated in a tangible product rather than ending in conversation alone. Many described catharsis or emotional release when hearing music that captured their personal experiences. Emotional shifts were observed as negative feelings such as sadness or frustration gave way to relief, joy, or greater objectivity depending on the music’s tone. Calm or soothing compositions promoted emotional clarity, while music visualization enhanced these effects by supporting sensory integration and revealing previously unrecognized emotions (n=11). Some (n=3) also gained a renewed sense of musical confidence and self-efficacy through this process.

\begin{quote}
\textit{``Because I have a simple way of thinking, I struggle to express emotions through words. But when music was added, I could feel and express them more richly.''} (P11)
\end{quote}
\begin{quote}
\textit{``Listening to a well-crafted piece that reflected my story helped me release negative emotions.''} (P23)
\end{quote}

\revised{\textbf{Mixed reactions when the music did not match users’ intent.} Several participants (n=7) reported that GenAI sometimes generated tracks did not fully match their intended mood or genre, which resulted in compositions that felt awkward, such as being \textit{``too bright''} or misaligned with their usual musical preferences. In these moments, a few participants (n=3) initially felt disappointed or sensed that the system did not fully understand their emotions. This temporarily weakened their sense of emotional resonance with the music. 
For example, P4 wrote to the CA about feeling exhausted and requested a calmer, more soothing song. However, the model returned a track that P4 experienced as heavier and more somber than expected, as if their request for \textit{``calm''} had been translated into \textit{``sad.''} Participants in such cases described a mismatch between \textit{``what I wrote” and \textit{``what I heard.''} However, many of the same participants later described these mismatches as opportunities to reflect on and reframe their feelings. Rather than dismissing the output, they used it to reconsider what they were actually experiencing or what kinds of sounds they might be open to.}} 

\begin{quote}
\textit{``I asked for calm music, but the result had a slightly different tone. Surprisingly, I liked it. It revealed something new about my musical taste.''} (P3)
\end{quote}

\begin{quote}
\textit{``I asked for calm music, but the result had a slightly different tone. Surprisingly, it helped me realize that what I was feeling wasn’t just calm. I think I was actually anxious underneath. It made me reflect more on how I really felt.''} (P5)
\end{quote}

\subsubsection{Reflective Dialogue and Discovery of Inner Resource after Music Appreciation}\hfill

\revised{\textbf{Discovery of inner resources and meaning through CA-guided song discussion.}} Design workshops with music therapists emphasized that the post-appreciative reflection phase is critical in transforming songwriting into a therapeutic process. In this study, all but three participants completed this phase, and our findings affirm its psychological value. Specifically, follow-up conversations with the CA after listening to their co-created music facilitated several cognitive shifts: (1) the rediscovery of personal strengths (P1, P5, P8), (2) reaffirmation of life values and purpose (P7, P11, P21, P23), and (3) reinterpretation of present circumstances through the lens of past experiences (P18, P20).

\begin{quote}
\textit{``When the chatbot asked, `What came to your mind during this part of the song?' I suddenly remembered why I started this journey and what my original goal was. It reminded me of the purpose of my life, which I had forgotten amid daily routines.''} (P11)
\end{quote}


The CA employed a structured strategy that began with prompts about favorite lyrics or musical segments and gradually transitioned into deeper reflections on emotional responses and evolving thought patterns. This stepwise conversation flow effectively supported participants in identifying core emotions and reconstructing personal meaning. Notably, the emotional engagement induced by appreciating their co-created music led some participants, especially those initially reserved, to open up more candidly. Two participants who had previously given vague or abstract responses were able to share more specific personal experiences during this phase, suggesting that music functioned as a mediating tool that reduced the discomfort of verbal disclosure and facilitated psychological openness through emotional activation (Table~\ref{tab: chat transcript-appreciation}).


\begin{table*}[t]
\begin{center}
  \caption{Chat transcript in our tool: Post-music appreciation inner work examples (P18 \& P20)}
  \label{tab: chat transcript-appreciation}
  \begin{tabular}{C{2cm} | C{2cm} |p{12cm}}
    \toprule
    \multicolumn{2}{c|}{Utterer} & Contents \\
    \midrule
    \multirow{1}{*}{P18} & Bot &  ``Parang, you mentioned feeling like you want to travel after listening to the song `Blue Sea Path Advance Party.' Was there a specific lyric or melody in this song that evoked this desire to travel?'' \\
    \hhline{~--}
    & User &  ``The part `Sing the song of the sea, move your feet to the rhythm of summer, refreshing waves' has an addictive melody.'' \\
    \hhline{~--}
    & Bot &  ``You said you liked the lyrics part `Sing the song of the sea, move your feet to the rhythm of summer, refreshing waves.' Is there a special place or moment that came to mind while listening to these lyrics?'' \\
    \hhline{~--}
    & User &  ``When I was in 6th grade, we planned a 10-day family trip to Jeju Island, and on the first day, I was having fun with my dad at the beach, but the next day, I fell off a cliff, so we had to urgently end the trip and go to a hospital. That memory comes back and feels nostalgic. It is a sad memory because it happened when I could not hear my dad’s voice well.''\\
    \hhline{~--}
    & Bot &  ``Such a nostalgic memory came to mind for you. Even as you recall that memory now, it seems you miss the time you spent with your dad at the beach. If you could go back to that sea now, what would you like to do?''\\
    \hhline{~--}
    & User &  ``Snorkeling with dad!''\\
    \midrule
    \multirow{1}{*}{P20} & Bot &  ``While listening to the song `Star of Dreams,' is there any lyrics that particularly resonate with you?''\\
    \hhline{~--}
    & User &  ``The moment sunshine illuminates my dream.''\\
    \hhline{~--}
    & Bot &  ``You said you liked the phrase `The moment sunshine illuminates my dream.' What feelings or thoughts come to mind when you hear this phrase?''\\
    \hhline{~--}
    & User &  ``Warmth and calmness.''\\
    \hhline{~--}
    & Bot &  ``You mentioned feeling warmth and calmness from the phrase `The moment sunshine illuminates my dream.' Is there any special memory or situation that comes to mind when you hear this phrase that you'd be willing to share?''\\
    \hhline{~--}
    & User &  ``I remember feeling good when I used to walk 10,000 steps while basking in the sunshine before my cochlear implant surgery, when I could not hear well.''\\
    \bottomrule
\end{tabular}

 \vspace{-10pt}
\end{center}
\end{table*}

\revised{\textbf{Limits in supporting emotional restructuring and therapeutic insight.}} However, several interactions revealed a limitation in eliciting emotional effects. The CA often rephrased emotional content without facilitating emotional restructuring, which refers to reframing and reorganizing emotions to generate new meanings and therapeutic insight, or supporting deeper self-structuring and personalized insight. Future tools should adopt advanced conversational frameworks that guide users through layered emotional journeys, from sensory awareness to emotional identification, associative memory, and meaning construction. Such designs could incorporate prompts that connect music to inner resources, promote positive recollection, and support therapeutic reflection and action.

\begin{quote}
\textit{``At first, it was hard to talk about my story in detail. But after listening to the music that captured my emotions, I felt more comfortable opening up. I think it’s because the music had already expressed my feelings.''} (P14)
\end{quote}
\begin{quote}
\textit{``I started crying while listening to the music. After that, I was able to talk to the chatbot much more honestly than at the beginning. The emotions I couldn’t express in words were captured in the music, which made it easier for me to speak about them.''} (P22)
\end{quote}

